Tsallis-thermometer: a QGP indicator for large and small collisional systems

The transverse momentum distribution of identified hadrons from recent years are analyzed within the thermodynamically consistent formulation of non-extensive statistics. A wide range of center-of-mass energies and average event multiplicities are studied for various hadron species. We demonstrate that the average event multiplicity is a key variable in the study of high-energy collisions and a smooth transition in the description from small to large systems is possible. For this purpose the non-extensive statistical approach is more than appropriate. The validity of the non-extensive description is explored in multiple ways: such as the calculation of integrated yields per unit rapidity, the analysis of radial flow and the consistency check of the thermodynamical variables. The 'Tsallis-thermometer' is introduced as an indicator of quark-gluon plasma in small collisional systems.

==> params/AuAu_200.tex <==
\begin{table}[H]
\caption{AuAu at $\sqrt{s_{NN}}=200$ GeV}
\label{tab:AuAu_02_lambdapm}
\begin{indented}
\item[]\begin{tabular}{@{}cccccc}
\br
    \textbf{Hadron} & $q$ & $T$ (GeV) & $A$ & $\chi^2/ndf$ \\
\mr
\textsc{\Lambda^0} & 1.080$\pm$0.005 & 0.200$\pm$0.008 & 4.17e-01$\pm$6.81e-02 & 307.38/39\\


==> params/CMe.tex <==
$\pi^\pm$ & $-0.543\pm0.235$ & $-1.047\pm0.082$ & $0.568\pm0.249$ & $563.798/6$\\ 
$K^\pm$ & $-0.429\pm1.124$ & $-1.278\pm1.093$ & $0.548\pm1.568$ & $463.932/6$\\ 
$p(\bar{p})$ & $0.105\pm1.034$ & $1.262\pm21.332$ & $0.132\pm21.357$ & $356.562/6$\\ 


==> params/Tqfits.tex <==
AuAu, 130 & $\pi^\pm$ & $0.655\pm0.086$ & $0.281\pm0.020$ & $0.184\pm0.088$ & $0.035/1$\\ 
  & $K^\pm$ & $0.624\pm0.052$ & $0.365\pm0.024$ & $0.228\pm0.057$ & $0.003/1$\\ 
  & $p(\bar{p})$ & $1.777\pm0.876$ & $0.157\pm0.077$ & $0.279\pm0.880$ & $0.262/1$\\ 
 AuAu, 200 & $\pi^\pm$ & $0.816\pm0.273$ & $0.256\pm0.050$ & $0.209\pm0.278$ & $0.436/2$\\ 
  & $K^\pm$ & $0.774\pm0.104$ & $0.313\pm0.038$ & $0.242\pm0.111$ & $0.073/2$\\ 
  & $p(\bar{p})$ & $1.070\pm0.163$ & $0.286\pm0.043$ & $0.306\pm0.168$ & $0.489/2$\\ 
  & CuCu, 200 & $K^0_s$ & $0.290\pm0.309$ & $0.694\pm0.651$ & $0.201\pm0.721$ & $1.049/3$\\ 
  & $\Phi$ & $1.114\pm0.182$ & $0.282\pm0.035$ & $0.315\pm0.186$ & $0.983/4$\\ 
  & $\Lambda^0$ & $1.330\pm0.164$ & $0.225\pm0.023$ & $0.299\pm0.166$ & $0.368/3$\\ 
  & $\Xi^{\pm}$ & $1.522\pm0.191$ & $0.222\pm0.023$ & $0.338\pm0.192$ & $0.284/3$\\ 
  & $\Omega^\pm$ & $1.066\pm0.087$ & $0.336\pm0.025$ & $0.358\pm0.090$ & $0.108/3$\\ 
 AuAu, 200 & $K^0_s$ & $0.782\pm0.181$ & $0.319\pm0.056$ & $0.250\pm0.189$ & $0.925/3$\\ 
  & $\Lambda^0$ & $1.509\pm0.088$ & $0.207\pm0.010$ & $0.312\pm0.088$ & $0.628/3$\\ 
 PbPb, 2760 & $\pi^\pm$ & $0.962\pm0.037$ & $0.261\pm0.005$ & $0.251\pm0.038$ & $4.703/8$\\ 
  & $K^\pm$ & $0.953\pm0.019$ & $0.322\pm0.005$ & $0.307\pm0.020$ & $3.031/8$\\ 
  & $K^0_s$ & $0.981\pm0.091$ & $0.316\pm0.018$ & $0.310\pm0.093$ & $2.361/5$\\ 
  & $K^{*0}$ & $1.129\pm0.758$ & $0.364\pm0.151$ & $0.411\pm0.773$ & $0.297/4$\\ 
  & $p(\bar{p})$ & $1.880\pm0.196$ & $0.216\pm0.022$ & $0.407\pm0.197$ & $160.411/8$\\ 
  & $\Phi$ & $1.135\pm0.290$ & $0.356\pm0.061$ & $0.404\pm0.296$ & $0.293/5$\\ 
  & $\Lambda^0$ & $1.939\pm0.116$ & $0.225\pm0.009$ & $0.437\pm0.116$ & $3.641/5$\\ 
  & $\Xi^{\pm}$ & $2.007\pm0.178$ & $0.217\pm0.017$ & $0.436\pm0.179$ & $0.629/3$\\ 
  & $\Omega^\pm$ & $0.937\pm0.142$ & $0.499\pm0.075$ & $0.468\pm0.160$ & $0.929/3$\\ 
 pPb, 5020 & $\pi^\pm$ & $3.340\pm0.414$ & $0.183\pm0.004$ & $0.610\pm0.414$ & $68.423/5$\\ 
  & $\pi^\pm$ (p) & $0.122\pm0.234$ & $1.000\pm1.543$ & $0.122\pm1.560$ & $140.018/5$\\ 
  & $K^\pm$ & $2.748\pm0.269$ & $0.215\pm0.007$ & $0.591\pm0.269$ & $78.110/5$\\ 
  & $K^\pm$ (p) & $1.715\pm0.319$ & $0.272\pm0.023$ & $0.467\pm0.320$ & $67.389/5$\\ 
  & $K^0_s$ (p) & $1.895\pm0.142$ & $0.248\pm0.009$ & $0.470\pm0.142$ & $17.055/5$\\ 
  & $K^{*0}$ & $2.437\pm0.241$ & $0.249\pm0.012$ & $0.606\pm0.241$ & $2.952/3$\\ 
  & $p(\bar{p})$ & $2.339\pm0.060$ & $0.220\pm0.003$ & $0.513\pm0.060$ & $5.950/5$\\ 
  & $p(\bar{p})$ (p) & $2.161\pm0.128$ & $0.229\pm0.008$ & $0.494\pm0.128$ & $9.400/5$\\ 
  & $\Phi$ & $2.779\pm0.221$ & $0.238\pm0.009$ & $0.662\pm0.221$ & $6.712/5$\\ 
  & $\Lambda^0$ (p) & $2.520\pm0.072$ & $0.213\pm0.003$ & $0.536\pm0.072$ & $2.242/5$\\ 
  & $\Xi^{\pm}$ & $1.983\pm0.257$ & $0.267\pm0.026$ & $0.530\pm0.259$ & $7.256/5$\\ 
  & $\Sigma^{\pm}$ & $2.321\pm0.750$ & $0.245\pm0.053$ & $0.569\pm0.752$ & $0.364/1$\\ 
  & $\Xi^0$ & $1.545\pm0.232$ & $0.333\pm0.048$ & $0.515\pm0.237$ & $1.818/2$\\ 
  & $\Omega^\pm$ & $1.815\pm0.390$ & $0.301\pm0.064$ & $0.545\pm0.395$ & $0.873/3$\\ 
 PbPb, 5020 & $\pi^\pm$ & $0.924\pm0.054$ & $0.273\pm0.008$ & $0.252\pm0.054$ & $5.935/8$\\ 
  & $K^\pm$ & $1.125\pm0.040$ & $0.305\pm0.006$ & $0.343\pm0.041$ & $7.058/8$\\ 
  & $p(\bar{p})$ & $2.048\pm0.029$ & $0.225\pm0.002$ & $0.460\pm0.029$ & $1.510/8$\\ 
 pp, 7000 & $\pi^\pm$ & $0.126\pm0.067$ & $1.000\pm2.084$ & $0.126\pm2.085$ & $1088.718/8$\\ 
  & $K^\pm$ & $5.792\pm3.096$ & $0.181\pm0.016$ & $1.047\pm3.096$ & $2766.136/8$\\ 
  & $K^0_s$ & $4.713\pm1.652$ & $0.187\pm0.014$ & $0.879\pm1.652$ & $576.128/8$\\ 
  & $K^{*0}$ & $3.799\pm0.512$ & $0.201\pm0.008$ & $0.762\pm0.512$ & $27.874/7$\\ 
  & $p(\bar{p})$ & $4.670\pm0.472$ & $0.173\pm0.005$ & $0.806\pm0.472$ & $97.376/8$\\ 
  & $\Phi$ & $3.257\pm0.409$ & $0.222\pm0.011$ & $0.723\pm0.409$ & $16.482/7$\\ 
  & $\Lambda^0$ & $3.113\pm0.075$ & $0.195\pm0.002$ & $0.606\pm0.075$ & $3.821/8$\\ 
  & $\Xi^{\pm}$ & $2.351\pm0.225$ & $0.226\pm0.012$ & $0.531\pm0.225$ & $7.821/8$\\ 
  & $\Omega^\pm$ & $2.208\pm0.885$ & $0.258\pm0.062$ & $0.571\pm0.888$ & $1.286/2$\\ 
 pp, 13000 & $K^0_s$ & $5.453\pm1.075$ & $0.186\pm0.007$ & $1.016\pm1.075$ & $545.854/8$\\ 
  & $\Lambda^0$ & $3.229\pm0.233$ & $0.197\pm0.006$ & $0.635\pm0.233$ & $30.657/8$\\ 
  & $\Xi^{\pm}$ & $2.755\pm0.353$ & $0.226\pm0.017$ & $0.622\pm0.353$ & $12.436/8$\\ 
  & $\Omega^\pm$ & $1.914\pm0.569$ & $0.309\pm0.074$ & $0.591\pm0.574$ & $1.467/3$\\ 
 

==> params/pp_13000.tex <==
\textsc{\Xi^\pm} & 1.134$\pm$0.001 & 0.490$\pm$0.015 & 1.91e-01$\pm$2.01e-05 & 382.66/10\\
\br
\end{tabular}
\end{indented}
\end{table}

